An Architectural Design for Measurement Uncertainty Evaluation in Cyber-Physical Systems

Several use cases from the areas of manufacturing and process industry, require highly accurate sensor data. As sensors always have some degree of uncertainty, methods are needed to increase their reliability. The common approach is to regularly calibrate the devices to enable traceability according to national standards and Syst\`eme international (SI) units - which follows costly processes. However, sensor networks can also be represented as Cyber Physical Systems (CPS) and a single sensor can have a digital representation (Digital Twin) to use its data further on. To propagate uncertainty in a reliable way in the network, we present a system architecture to communicate measurement uncertainties in sensor networks utilizing the concept of Asset Administration Shells alongside methods from the domain of Organic Computing. The presented approach contains methods for uncertainty propagation as well as concepts from the Machine Learning domain that combine the need for an accurate uncertainty estimation. The mathematical description of the metrological uncertainty of fused or propagated values can be seen as a first step towards the development of a harmonized approach for uncertainty in distributed CPSs in the context of Industrie 4.0. In this paper, we present basic use cases, conceptual ideas and an agenda of how to proceed further on.

==> Makefile <==
-include lib/resources/build/Makefile

fixme:
	@echo "Seems you forgot the checkout the 'lib' using the recursive parameter."
	@echo "Fixing it for you..."
	@git submodule update --init --recursive || git clone https://github.com/tubav/Core.git lib

.PHONY: html

no-acro:
	@grep -Eo "^\s*[^%][^{=]*[A-Z]{2,}" src/*.tex

html:
	@echo "TODO: move to library"
	@echo "TODO: fix issues with subfigures"
	@echo "TODO: fix issues with index"
	@echo "TODO: enhance 'make clean'"
	@echo "TODO: mention 'tlmgr install make4ht tex4ht'"
	pdflatex template
	pdflatex template
	biber template
	pdflatex template
	make4ht -u -d html template "htmlimages,htmlcolor,html5,charset=utf-8,fn-in"
	perl -i -0pe 's/<img.*\n.*alt="PICT".*//g' html/template.html
	perl -i -0pe 's/<hr class=".*figure".*\/>//g' html/template.html
	perl -i -0pe 's/<\?.*\n.*\n.*\n.*\n//' html/template.html


==> lib/resources/build/Makefile <==
SHELL = bash
.PHONY: overleaf

help:
	@echo " * clean     : Delete temporary files"
	@echo " * all       : Create the PDF file (run everything needed)"
	@echo " * full      : Create the PDF file (run LaTeX and BibTeX only)"
	@echo " * quicker   : Update the PDF file (just run LaTeX twice)"
	@echo " * quick     : Update the PDF file (just run LaTeX once)"
	@echo " * deps      : Download LaTeX dependencies"
	@echo " * bib       : Update the bib file (just run BibTeX/biber once)"
	@echo " * bibchk    : Run some checks (e.g. biber, bibtex-check)"
	@echo " * verify    : Run some checks (e.g. l2tabu)"
	@echo " * spell     : Check for spelling errors (aspell)"
	@echo " * eval      : Run evaluation scripts (e.g. R)"
	@echo " * generate  : Generate images (gnuplot, R, dot/graphviz, ...)"
	@echo " * deploy    : Deploy the PDF file to a directory (e.g. for automated builds)"
	@echo " * update    : Get the latest sources (incl. latest library)"
	@echo " * open      : Opens the output file using 'open'"
	@echo " * ci        : Continuous Integration - watch for changes an rebuild everything"
	@echo " * rename    : Rename project"
	@echo " * unicode   : Find incompatible unicode characters"
	@echo " * optimize  : Optimize output (e.g. optipng)"
	@echo " * sign      : Sign the PDF using an X.509 certificate"
	@echo " * preflight : Test for PDF/A and PDF/X compatibility"
	@echo " * fix       : Try to fix some common issues (file encoding, biber cache, ...)"
	@echo " * todo      : Find open todos"
	@echo " * debug     : Compile and stop on error and show line number"
	@echo " * updating  : Keep updating in the background to avoid conflicts"
	@echo " * ieee      : Enable IEEE Transaction style"
	@echo " * llncs     : Enable LLNCS style"
	@echo " * content   : Answer basic questions to bootstrap your paper"
	@echo " * count     : Count number of words, figures, tables, captions, ..."
	@echo " * overleaf  : Open project in overleaf (if overleaf is used)"

OID = $(shell grep 'url' .git/config|grep 'overleaf'|awk -F "/" '{print $$4}')
overleaf:
ifeq ($(strip $(OID)),)
	@echo "Seems overleaf is not being used"
else
	@open https://www.overleaf.com/project/$(OID)
endif

count:
	@echo "Counting..."
	@command -v texcount >/dev/null 2>&1 || { echo >&2 "ERROR: run 'tlmgr install texcount' first."; exit 1; }
	@texcount -nosub -total -utf8 -letter src/*.tex

ieee:
	@echo "Changing to IEEE Transaction style..."
	@find . -maxdepth 1 -type f -iname "*.tex" -exec perl -p -i -e 's/([\s])*%+([^%]*)(% enable for IEEE style)/\1\2\3/g' {} \; -exec perl -p -i -e 's/([\s])*([^%]*)(% enable for LLNCS style)/\1%\2\3/g' {} \;

llncs:
	@echo "Changing to LLNCS Transaction style..."
	@find . -maxdepth 1 -type f -iname "*.tex" -exec perl -p -i -e 's/([\s])*%+([^%]*)(% enable for LLNCS style)/\1\2\3/g' {} \; -exec perl -p -i -e 's/([\s])*([^%]*)(% enable for IEEE style)/\1%\2\3/g' {} \;

content:
	@read -p "Area: one sentence about the research area (which broad area are we considering?): " area; \
	read -p "Issue: one sentence about the issue (what issue is getting to get solved?): " issue; \
	read -p "Related Work: one sentence about the shortcomings of existing solutions: " related; \
	read -p "Assumptions: made in general terms. In this paper, we assume ... : " assumptions; \
	read -p "Approach: one sentence about the own approach: " approach; \
	read -p "Validation: one sentence about the validation of the results. We have validated our approach by...: " validation; \
	read -p "Result: one sentence about the main contribution. The main contribution of this paper is...: " result; \
	perl -p -i -e "s/.*%%area/$$area. %%area/g" src/00_abstract.tex; \
	perl -p -i -e "s/.*%%issue/$$issue. %%issue/g" src/00_abstract.tex; \
	perl -p -i -e "s/.*%%related/$$related. %%related/g" src/00_abstract.tex; \
	perl -p -i -e "s/.*%%assumptions/$$assumptions. %%assumptions/g" src/00_abstract.tex; \
	perl -p -i -e "s/.*%%approach/$$approach. %%approach/g" src/00_abstract.tex; \
	perl -p -i -e "s/.*%%validation/$$validation. %%validation/g" src/00_abstract.tex; \
	perl -p -i -e "s/.*%%result/$$result. %%result/g" src/00_abstract.tex; \
	perl -p -i -e "s/.*%%area/\\\todotext{$$area}%%area/g" src/01_introduction.tex; \
	perl -p -i -e "s/.*%%issue/\\\todotext{$$issue}%%issue/g" src/01_introduction.tex; \
	perl -p -i -e "s/.*%%related/\\\todotext{$$related}%%related/g" src/01_introduction.tex; \
	perl -p -i -e "s/.*%%assumptions/In this paper, we assume \\\todotext{$$assumptions}%%assumptions/g" src/01_introduction.tex; \
	perl -p -i -e "s/.*%%approach/\\\todotext{$$approach}%%approach/g" src/01_introduction.tex; \
	perl -p -i -e "s/.*%%validation/We have validated our approach by \\\todotext{$$validation}%%validation/g" src/01_introduction.tex; \
	perl -p -i -e "s/.*%%result/The main contribution of this paper is \\\todotext{$$result}%%result/g" src/01_introduction.tex

updating:
	@while true; do $(MAKE) update; sleep 30; done

fixmod:
	@chmod +x build.sh

debug: fixmod
	@./build.sh -y

todo:
	@find src -iname "*.tex" -exec sh -c "grep -Hin 'TODO{' {}|sed 's/^\(.*\):\(.*\):.*{\(.*\)}/ * TODO \"\3\" in file \1 in line \2/'" \;

clean: fixmod
	@./build.sh -c

all: generate fixmod
	@./build.sh -b

full: fixmod
	@./build.sh -b

quick: fixmod
	@./build.sh -q

quicker: fixmod
	@./build.sh -r

deps: fixmod
	@./build.sh -t

bib: fixmod
	@./build.sh -i

bibchk: fixmod
	@./build.sh -w

verify: fixmod
	@./build.sh -v

spell: fixmod
	@./build.sh -s

eval: fixmod
	@./build.sh -e

generate: fixmod
	@./build.sh -g

open: fixmod
	@./build.sh -o

deploy: fixmod
	@./build.sh -d ${DPATH}

ci: fixmod
	@./build.sh -f

unicode: fixmod
	@./build.sh -u

optimize: fixmod
	@./build.sh -z

sign: fixmod
	@./build.sh -x

preflight: fixmod
	@./build.sh -p

rename: fixmod
	@./build.sh -n

fix:
	@echo -n "Removing biber cache..."; rm -rf "$(shell biber --cache)"; echo "done"
	@echo -n "Normalizing Unicode..."; ./build.sh -m; echo "done"
	@make clean

update:
	@git submodule foreach git pull origin master
	@git pull


==> lib/resources/config/default.tex <==
% bugfixes ---------------------------------------------------------------------
%\let\spvec\vec                   % llncs with amsmath bugfix
%\let\vec\accentvec               % llncs with amsmath bugfix
%\newcommand{\subparagraph}{}     % IEEETrans with titlesec bugfix

%\makeatletter                    % for old listings package
%\@ifundefined{float@listhead}{}{%
%    \renewcommand*{\lstlistoflistings}{%
%        \begingroup
%            \if@twocolumn
%                \@restonecoltrue\onecolumn
%            \else
%                \@restonecolfalse
%            \fi
%            \float@listhead{\lstlistlistingname}%
%            \setlength{\parskip}{\z@}%
%            \setlength{\parindent}{\z@}%
%            \setlength{\parfillskip}{\z@ \@plus 1fil}%
%            \@starttoc{lol}%
%            \if@restonecol\twocolumn\fi
%        \endgroup
%    }%
%}
%\makeatother
% ------------------------------------------------------------------------------

% macro: ifpackageloaded -------------------------------------------------------
\makeatletter
\providecommand{\IfPackageLoaded}[2]{\@ifpackageloaded{#1}{#2}{}}
\providecommand{\IfPackageNotLoaded}[2]{\@ifpackageloaded{#1}{}{#2}}
\providecommand{\IfElsePackageLoaded}[3]{\@ifpackageloaded{#1}{#2}{#3}}
\makeatother
% ------------------------------------------------------------------------------

% File encoding: Normal UTF8 ---------------------------------------------------
\IfPackageNotLoaded{CJKutf8}{\usepackage[utf8]{inputenc}}
\usepackage[T1]{fontenc}     % Font encoding: T1
%\usepackage{cmap}           % Support copy and search for pdflatex
\input{glyphtounicode}       % Support copy and search for pdflatex % chktex 27
%\pdfgentounicode=1          % Support copy and search for pdflatex
\makeatletter
\def\UTFviii@defined#1{%
  \ifx#1\relax
      ((TODO:\@ Fix weird character here))%
  \else\expandafter% chktex 41
    #1%
  \fi
}
\makeatother
% ------------------------------------------------------------------------------

% ------------------------------------------------------------------------------
\usepackage{amssymb}                  % Springer Verlag (pdflatex)
\makeatletter
\@ifpackageloaded{url}{}{\usepackage[hyphens]{url}} % Create URLs in the document
\makeatother
\usepackage[
spacing=true,                         % Fonts: spacing?
kerning=true,
tracking=true,                        % Fonts: hyphenatable letterspacing
expansion=true,                       % Fonts: better grey value
protrusion=true]{microtype}           % Fonts: margin kerning
\microtypecontext{spacing=nonfrench}
\usepackage{textcomp}                 % For the Euro sign
\usepackage{booktabs}                 % Nice tables
\usepackage{listings}                 % Nice listings
\usepackage{listingsutf8}             % Listings with UTF-8
\lstset{columns=fullflexible,         % Listings in multicolumn mode
        breaklines=true,              % Listings with long lines
        xleftmargin=3em,              % Correct indentation
        basicstyle=\scriptsize,       % Small text
        numbers=left,                 % Show numbers
        stepnumber=1,                 % For each line
        inputencoding=utf8            % Enable UTF8
        }
\usepackage{algorithmic}              % Nice pseudo code
\makeatletter
\@ifpackageloaded{tex4ht}{%
  \usepackage[dvipdfmx]{color,graphicx}
}{
  \usepackage[table]{xcolor}                   % To use and define colors
  \usepackage{subcaption}               % Subfigures
}
\makeatother
\definecolor{LinkColor}{rgb}          % Link color
{0.31,0.46,.64}                       %
\definecolor{MarginColor}{rgb}        % Margin color
{0.31,0.46,.64}                       %
\usepackage{wrapfig}                  % Use floating images
\usepackage{stfloats}                 % Makes LaTeX honour ‘[b]’ placement
\usepackage{amsmath}                  % For eqref
\usepackage[olditem,oldenum]{paralist}% For inline lists (options for MDPI)
%\usepackage{fixltx2e}                 % Provides fixes for LaTeX (not needed for anymore since 2015)
\usepackage{fix-cm}                   % Provides fixes for LaTeX
\usepackage{rotating}                 % e.g. for the special side margin notes
\usepackage{lipsum}                   % To add some dummy text
\usepackage{xspace}                   % Fixing some spacing issues
\usepackage{ellipsis}                 % Puts space around ellipses
%\usepackage{ragged2e}                 % New commands/env. for setting ragged text
%\usepackage{lmodern}                 % Nicer fonts (for all)
\usepackage{ltxtable}                 % Long complex tables
\usepackage{ltablex}                  % Long complex tables
\newcolumntype{L}{>{\raggedright\arraybackslash}X}
\makeatletter
\@ifpackageloaded{lineno}{}{\usepackage[switch*,modulo]{lineno}}   % Show line numbers
\makeatother
\makeatletter
\@ifpackageloaded{accsupp}{}{\usepackage{accsupp}} % Don't copy line numbers (see below)
\makeatother
\renewcommand{\thelinenumber}{        % Line number printing mechanism
  \BeginAccSupp{ActualText={}}\arabic{linenumber}\EndAccSupp{}%
}
\usepackage{blindtext}                % insert blind texts
%\usepackage{cleveref}                 % To ref footnotes twice (use after hyperref)
%\crefformat{footnote}{#2\footnotemark[#1]#3}

\makeatletter
\newcommand*{\etc}{%
    \@ifnextchar{.}%
        {etc}%
        {etc.\@\xspace}%
}
\makeatother
\newcommand*{\eg}{e.g.\@\xspace}
\newcommand*{\ie}{i.e.\@\xspace}
\newcommand*{\cf}{cf.\@\xspace}
\newcommand*{\zB}{z.\,B.\@\xspace}
\newcommand*{\zT}{z.\,T.\@\xspace}
\newcommand*{\ddh}{d.\,h.\@\xspace}
\newcommand*{\va}{v.\,a.\@\xspace}
\newcommand*{\ua}{u.\,a.\@\xspace}
\newcommand*{\uU}{u.\,U.\@\xspace}
\newcommand*{\zZ}{z.\,Z.\@\xspace}
\newcommand*{\bzw}{bzw.\@\xspace}
\newcommand*{\bspw}{bspw.\@\xspace}
\newcommand*{\ggf}{ggf.\@\xspace}
\newcommand*{\vgl}{vgl.\@\xspace}

% To be used in the project specific config file:
%\usepackage[bf]{caption}[2008/08/24]  % Bold caption (better contrast)
%\usepackage{acronym}                  % For acronyms
%\usepackage[pdftex]{graphicx}         % Include images for pdflatex

\hyphenation{op-tical net-works semi-conduc-tor con-cept}

\renewcommand{\figurename}{Fig.}
\renewcommand{\tablename}{Tab.}
\newcommand{\sectionname}{Sec.}
\newcommand{\equationname}{Eq.}
\renewcommand{\lstlistlistingname}{List of Listings}

\makeindex

\setcounter{tocdepth}{3}
\newcommand{\mykeywords}[1]{\par\addvspace\baselineskip%
\keywordname\enspace\ignorespaces#1}
\makeatletter
\providecommand*{\toclevel@title}{99}
\providecommand*{\toclevel@author}{99}

\usepackage[tocindentauto]{tocstyle}      % fixing large roman page letters in ToC
\usetocstyle{standard}                    % same layout as before
\settocstylefeature{pagenumberbox}{\hbox} % fixing large roman page letters in ToC
% type setting ----------------------------------------------------------------
% no "Schusterjungen"
    \clubpenalty=10000
% no "Hurenkinder"
    \widowpenalty=10000
    \displaywidowpenalty=10000
% type setting ----------------------------------------------------------------

% annotations --------------------------------------------------------------
\newcommand{\annot}[2][]{%
    \pdfannot\ width \linewidth\ height 2\baselineskip\ depth 0pt{%
        /Subtype/Text%
        /Open false
        /Name /Comment%
        /CA .4%
        /C [.3 .6 .9]%
        /T (\pdfescapestring{#1})%            /Contents(\pdfescapestring{\detokenize{#2}})%
    }
}

\newcommand\acc[1]{%
{%
\renewcommand{\url}[1]{}%
\renewcommand{\footnote}[1]{}%
\renewcommand{\cite}[1]{}%
\renewcommand{\nobreakspace}{}%
\let\protect\relax%
\ac*{#1}%
}%
}
\newcommand\aclc[1]{%
{%
\renewcommand{\url}[1]{}%
\renewcommand{\footnote}[1]{}%
\renewcommand{\cite}[1]{}%
\renewcommand{\nobreakspace}{}%
\let\protect\relax%
\acl*{#1}%
}%
}
\newcommand\acfc[1]{%
{%
\renewcommand{\url}[1]{}%
\renewcommand{\footnote}[1]{}%
\renewcommand{\cite}[1]{}%
\renewcommand{\nobreakspace}{}%
\let\protect\relax%
\acf*{#1}%
}%
}
\newcommand\todoremark[1]{%
	\color{blue}%
	((remark: #1))
	\color{black}%
}
\newcommand\todo[1]{%
	\color{red}%
	((todo: #1))
	\color{black}%
}
\newcommand\todotext[1]{%
    \todo{#1}%
	\color[gray]{0.8}%
	\blindtext[1]
	\color{black}%
}

\newcommand\todowrite[2]{%
  \color{red}%
  ((write about #1))
	\color[gray]{0.8}%
	Lorem ipsum dolor sit amet, consectetur adipisicing elit, sed do eiusmod tempor incididunt ut labore et dolore magna aliqua. Ut enim ad minim veniam, quis nostrud exercitation ullamco laboris nisi ut aliquip ex ea commodo consequat. Duis aute irure dolor in reprehenderit in voluptate velit esse cillum dolore eu fugiat nulla pariatur.
  #2
	\color{black}%
}


\newcommand\todosmall[1]{%
    \todo{#1}%
	\color[gray]{0.8}%
	Lorem ipsum dolor sit amet, consectetuer adipiscing elit. Etiam lobortis facilisis sem. Nullam nec mi et neque pharetra sollicitudin. Praesent imperdiet mi nec ante.
	\color{black}%
}
\newcommand\todoshort[1]{\todosmall{#1}}
\newcommand\todomid[1]{%
    \todo{#1}%
    \color[gray]{0.8}%
    Lorem ipsum dolor sit amet, consectetur adipisicing elit, sed do eiusmod tempor incididunt ut labore et dolore magna aliqua. Ut enim ad minim veniam, quis nostrud exercitation ullamco laboris nisi ut aliquip ex ea commodo consequat. Duis aute irure dolor in reprehenderit in voluptate velit esse cillum dolore eu fugiat nulla pariatur.
    \color{black}%
}

\usepackage{ifoddpage}                % Move notes to correct page
\usepackage{needspace}                % Avoid hanging notes
\usepackage{marginnote,zref-savepos}  % Non floating margin notes

%\setlength{\marginparwidth}{0.7in}
\newcommand\sidenote[1]{\mbox{}%
  \marginnote{%
    \scriptsize%
    %\raggedright%
    \hspace{0pt}%
    \color{MarginColor}%
    %\begin{turn}{270}%
      \emph{#1}%
    %\end{turn}%
  }%
}%
\makeatletter
\@ifpackageloaded{tex4ht}{\renewcommand\sidenote[1]{}}{}
\makeatother

% annotations --------------------------------------------------------------

% more listings ------------------------------------------------------------
\definecolor{grey}{rgb}{0.5,0.5,0.5}
\lstdefinelanguage{sparql}{
morecomment=[l][\color{black}]{\#},
morestring=[b][\color{black}]\",
morekeywords={SELECT,CONSTRUCT,DESCRIBE,ASK,WHERE,FROM,NAMED,PREFIX,BASE,OPTIONAL,FILTER,GRAPH,LIMIT,OFFSET,SERVICE,UNION,EXISTS,NOT,BINDINGS,MINUS,a},
sensitive=true
}
\lstdefinelanguage{ttl}{
sensitive=true,
morecomment=[l][\color{grey}]{@},
morecomment=[l][\color{black}]{\#},
morestring=[b][\color{black}]\",
}
\definecolor{groovyblue}{rgb}{0,0,.9}
\definecolor{groovygreen}{rgb}{0,.7,0}
\definecolor{darkgray}{rgb}{.4,.4,.4}

\lstdefinelanguage{Groovy}[]{Java}{
  keywordstyle=\color{groovyblue}\bfseries,
  stringstyle=\color{groovygreen}\ttfamily,
  keywords=[3]{each, findAll, groupBy, collect, inject, eachWithIndex},
  morekeywords={def, as, in, use},
  moredelim=[is][\textcolor{darkgray}]{\%\%}{\%\%}, % chktex 21
  moredelim=[il][\textcolor{darkgray}]{§§}
}
% more listings ------------------------------------------------------------

% show the hex code of the unknown unicode character to actually find it ----
\usepackage{stringenc}
\usepackage{pdfescape}
\makeatletter
\renewcommand*{\UTFviii@defined}[1]{%
  \ifx#1\relax
    \begingroup
      % Remove prefix "\u8:"
      \def\x##1:{}%
      % Extract Unicode char from command name
      % (utf8.def does not support surrogates)
      \edef\x{\expandafter\x\string#1}% chktex 41
      \StringEncodingConvert\x\x{utf8}{utf16be}% convert to UTF-16BE
      % Hexadecimal representation
      \EdefEscapeHex\x\x
      % Enhanced error message
      \PackageError{inputenc}{Unicode\space char\space \string#1\space
                              (U+\x)\MessageBreak%
                              not\space set\space up\space
                              for\space use\space with\space LaTeX}\@eha%
    \endgroup
  \else\expandafter% chktex 41
    #1%
  \fi
}
\makeatother
% ---------------------------------------------------------------------------

% own requirement environment --------------------------------------------------
\makeatletter
\newcommand\requirement[3]{%
  \protected@write\@auxout{}{\string\CreateCounter{#1}}% chktex 21
  \crefname{my#1}{requirement}{requirements}\Crefname{my#1}{Requirement}{Requirements} %fixme:doesn't work
  \crefname{#1}{requirement}{requirements}\Crefname{#1}{Requirement}{Requirements} %fixme:doesn't work
  \@ifundefined{c@my#1}
    {#1??: #3}
    {\refstepcounter{my#1}\label{#2}#1\arabic{my#1}: #3}%
}
\newcommand{\CreateCounter}[1]{%
  \@ifundefined{c@my#1}
    {\newcounter{my#1}\global\@namedef{themy#1}{#1\arabic{my#1}}}% chktex 21
    {}%
}
\AtEndDocument{\let\CreateCounter\@gobble}% chktex 21
\makeatother
% ------------------------------------------------------------------------------


==> src/04_evaluation.tex <==
%\section{Evaluation: Scalability of the Current Implementation}\label{sec:evaluation}
\section{Evaluation}\label{sec:evaluation} 
%-------------------------------------------------------------------------------
%Evaluation: How does it really work in practice? Provide real or simulated
%performance metrics, end-user studies, mention external technology adoptors,
%if any, etc.

%This section presents the detailed results you have obtained. If the paper
%is theoretical, you might want to show curves obtained from your equations.
%If the paper is experimental, you will be presenting curves showing the
%measurement results. In order to choose the proper curves to present, you
%must first be clear what point you are trying to convey to the reader. The 
%curves can then be chosen to illustrate this point. Whether your paper is
%theoretical or experimental, you must provide a careful interpretation of
%what your results mean and why they behave as they do.
%-------------------------------------------------------------------------------
% This section presents the detailed results obtained. It contains the results
% obtained from the analytical model, the emulations and the simulations realized
% as well as the interpretation and discussion of them. 
%-------------------------------------------------------------------------------
% The goals of the study,
% The system boundaries
% System services and possible outcomes
% Selected performance metrics
% System and workload parameters
% Factors and their values
% Evaluation techniques
% Selected workload
% Design of the experiments
% Analysis and interpretation of the data
% Presentation of the results
%------------------------------------------------------------------------------_

Evaluation: How does it really work in practice? Provide real or simulated
performance metrics, end-user studies, mention external technology adopters,
if any, and so on.

This section presents the detailed results you have obtained. If the paper
is theoretical, you might want to show curves obtained from your equations.
If the paper is experimental, you will be presenting curves showing the
measurement results. In order to choose the proper curves to present, you
must first be clear what point you are trying to convey to the reader. The 
curves can then be chosen to illustrate this point. Whether your paper is
theoretical or experimental, you must provide a careful interpretation of
what your results mean and why they behave as they do.

See \Cref{fig:example1} and \Cref{fig:example2}.

\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{resources/images/example1.pdf} 
    \caption{Example image.}\label{fig:example1}
\end{figure}

\begin{figure}
    \begin{subfigure}[b]{.5\textwidth}
    	\centering
		\includegraphics[width=.5\textwidth]{resources/images/example2.pdf}
		\caption{Example2}\label{fig:example2}
    \end{subfigure}
    \begin{subfigure}[b]{.5\textwidth}
    	\centering
		\includegraphics[width=.5\textwidth]{resources/images/example3.pdf}
		\caption{Example3}\label{fig:example3}
    \end{subfigure}    
    \caption{Example images.}\label{fig:exammple2_3}
\end{figure}


==> stuff/2020.famous.reqs.acro.tex <==
\DeclareAcronym{AAS}{short={AAS}, long={Asset Administration Shell}}
\DeclareAcronym{Bosch}{short={Bosch}, long={Robert Bosch GmbH}}
\DeclareAcronym{CPS}{short={CPS}, long={Cyber Physical Systems}}
\DeclareAcronym{DT}{short={DT}, long={Digital Twin}}
\DeclareAcronym{E+H}{short={E+H}, long={Endress+Hauser SE \& Co KG}}
\DeclareAcronym{EC}{short={EC}, long={Edge Computing}}
\DeclareAcronym{FAMOUS}{short={FAMOUS}, long={AAS-based modeling for the analysis of mutable CPS}}
\DeclareAcronym{Greedy Computing}{short={Greedy Computing}, long={Greedy Computing}, cite={Foster:2004}}
\DeclareAcronym{I40}{short={I4.0}, long={Industrie 4.0}}
\DeclareAcronym{IIoT}{short={IIoT}, long={Industrial Internet of Things}}
\DeclareAcronym{IPK}{short={IPK}, long={Fraunhofer Institute for Production Systems and Design Technology}}
\DeclareAcronym{IT}{short={IT}, long={Information Technology}}
\DeclareAcronym{ML}{short={ML}, long={Machine Learning}}
\DeclareAcronym{NMI}{short={NMI}, long={National Metrology Institute}}
\DeclareAcronym{OC}{short={OC}, long={Organic Computing}}
\DeclareAcronym{OT}{short={OT}, long={Operation Technology}}
\DeclareAcronym{OPC}{short={OPC UA}, long={Open Platform Communications United Architecture}}
\DeclareAcronym{SI}{short={SI}, long={Système International}}
\DeclareAcronym{API}{short={API}, long={Application Programming Interface}}
\DeclareAcronym{PTP}{short={PTP}, long={Precision Time Protocol}}


==> stuff/2020.famous.reqs.meta.tex <==
% existing authors list --------------------------------------------------------
\IfFileExists{global-do-not-edit.authors.tex}{\input{global-do-not-edit.authors.tex}}{} % chktex 27
% ------------------------------------------------------------------------------


% authors ----------------------------------------------------------------------
\newcommand{\metaAuthorWenzel}{Wenzel Pilar von Pilchau}
\newcommand{\metaMailWenzel}{wenzel.pilar-von-pilchau@informatik.uni-augsburg.de}
\newcommand{\metaInstWenzel}{University of Augsburg, Augsburg, Germany, \\Organic Computing Group}

\newcommand{\metaAuthorMRI}{Matthias Riedl}
\newcommand{\metaMailMRI}{matthias.riedl@ifak.eu}
\newcommand{\metaInstMRI}{ifak e.V., Magdeburg, Germany,\\ICT \& Automation}

\newcommand{\metaAuthorMG}{Maximilian Gruber}
\newcommand{\metaMailMG}{maximilian.gruber@ptb.de}
\newcommand{\metaInstMG}{PTB, Berlin, Germany,\\Presidential Staff}

\newcommand{\metaAuthorJT}{Jawad Tayyub}
\newcommand{\metaMailJT}{jawad.tayyub@endress.com}
\newcommand{\metaInstJT}{Endress + Hauser, Maulburg, Germany,\\Technology Development}

\newcommand{\metaAuthorNK}{Nikolaos-Stefanos Koutrakis}
\newcommand{\metaMailNK}{nikolaos-stefanos.koutrakis@ipk.fraunhofer.de}
\newcommand{\metaInstNK}{Fraunhofer IPK, Berlin, Germany,\\Production Machines and System Management}

\newcommand{\metaAuthorVG}{Varun Gowtham}
\newcommand{\metaMailVG}{varun.gowtham@fokus.fraunhofer.de}
\newcommand{\metaInstVG}{Fraunhofer FOKUS, Berlin, Germany,\\Open Communication Systems}

% ------------------------------------------------------------------------------

% author PDF -------------------------------------------------------------------
\newcommand{\metaAuthorMail}{\metaMailFirst}
\newcommand{\metaAuthorShort}{\metaAuthorFirst}
% ------------------------------------------------------------------------------

% author IEEE ------------------------------------------------------------------
\newcommand{\IEEEinstFirst}{\IEEEauthorblockA{\metaInstFirst}} % enable for IEEE style
\newcommand{\IEEEauthorFirst}{\IEEEauthorblockN{\metaAuthorFirst}\IEEEinstFirst} % enable for IEEE style

\newcommand{\IEEEinstWenzel}{\IEEEauthorblockA{\metaInstWenzel}} % enable for IEEE style
\newcommand{\IEEEauthorWenzel}{\IEEEauthorblockN{\metaAuthorWenzel}\IEEEinstWenzel} % enable for IEEE style

\newcommand{\IEEEinstMRI}{\IEEEauthorblockA{\metaInstMRI}} % enable for IEEE style
\newcommand{\IEEEauthorMRI}{\IEEEauthorblockN{\metaAuthorMRI}\IEEEinstMRI} % enable for IEEE style

\newcommand{\IEEEinstMG}{\IEEEauthorblockA{\metaInstMG}} % enable for IEEE style
\newcommand{\IEEEauthorMG}{\IEEEauthorblockN{\metaAuthorMG}\IEEEinstMG} % enable for IEEE style

\newcommand{\IEEEinstJT}{\IEEEauthorblockA{\metaInstJT}} % enable for IEEE stylehttps://www.overleaf.com/project/5e58de38377fd900013f9c1b
\newcommand{\IEEEauthorJT}{\IEEEauthorblockN{\metaAuthorJT}\IEEEinstJT} % enable for IEEE style

\newcommand{\IEEEinstNK}{\IEEEauthorblockA{\metaInstNK}} % enable for IEEE style
\newcommand{\IEEEauthorNK}{\IEEEauthorblockN{\metaAuthorNK}\IEEEinstNK} % enable for IEEE style

\newcommand{\IEEEinstVG}{\IEEEauthorblockA{\metaInstVG}} % enable for IEEE style
\newcommand{\IEEEauthorVG}{\IEEEauthorblockN{\metaAuthorVG}\IEEEinstVG} % enable for IEEE style


\author{
 \IEEEauthorblockN{\\
        \parbox{\linewidth}{\centering
            Wenzel Pilar von Pilchau\IEEEauthorrefmark{1},
            Varun Gowtham\IEEEauthorrefmark{6},
            Maximilian Gruber\IEEEauthorrefmark{3},
            Matthias Riedl\IEEEauthorrefmark{2},
            Nikolaos-Stefanos Koutrakis\IEEEauthorrefmark{5},
            Jawad Tayyub\IEEEauthorrefmark{4},
            Jörg Hähner\IEEEauthorrefmark{1},
            Sascha Eichstädt\IEEEauthorrefmark{3},
            Eckart Uhlmann\IEEEauthorrefmark{5},
            Julian Polte\IEEEauthorrefmark{5},
            Volker Frey\IEEEauthorrefmark{4} and
            Alexander Willner\IEEEauthorrefmark{6}
        }
    }
    \and
    \IEEEauthorblockA{\IEEEauthorrefmark{1}University of Augsburg, Augsburg, Germany,\\Organic Computing Group}
    \and
    \IEEEauthorblockA{\IEEEauthorrefmark{3}PTB, Berlin, Germany,\\Presidential Staff}
    \and
    \IEEEauthorblockA{\IEEEauthorrefmark{5}Fraunhofer IPK, Berlin, Germany,\\Production Machines and System Management}
    \and
    \IEEEauthorblockA{\IEEEauthorrefmark{2}ifak e.V., Magdeburg, Germany,\\ICT \& Automation}
    \and
    \IEEEauthorblockA{\IEEEauthorrefmark{4}Endress + Hauser, Maulburg, Germany,\\Technology Development}
    \and
    \IEEEauthorblockA{\IEEEauthorrefmark{6}Fraunhofer FOKUS, Berlin, Germany,\\Open Communication Systems}

} % enable for IEEE style
% ------------------------------------------------------------------------------

% author LLNCS -----------------------------------------------------------------
%\author{\metaAuthorFirst\inst{1} \and \metaAuthorWillner\inst{2}\inst{3}} % enable for LLNCS style
%\authorrunning{\metaAuthorFirst et al.} % enable for LLNCS style
%\tocauthor{\metaAuthorFirst, \metaAuthorXXX} % enable for LLNCS style
%\institute{\metaInstFirst\\ % enable for LLNCS style
%\email{\metaMailFirst} % enable for LLNCS style
%\and \metaInstFOKUS\\\email{\metaMailWillnerFOKUS} \\ % enable for LLNCS style
%\and \metaInstTUB\\\email{\metaMailWillnerTUB}% enable for LLNCS style
%} % enable for LLNCS style
%\titlerunning{\metaTitleShort} % enable for LLNCS style
% ------------------------------------------------------------------------------

\newcommand{\metaThanks}{Research for this paper %
was financed by the Federal Ministry of Education and Research (BMBF) project %
FAMOUS\footnote{\url{http://famous-project.eu/}}.
%\cite{rfc748}\todo{is there an official reference? MRI: Foerderkennzeichen 01|S18078}.
We thank our project partners for their contributions and their collaboration to this research work.}
% ------------------------------------------------------------------------------

